Low-rank extended Kalman filtering for online learning of neural networks from streaming data

We propose an efficient online approximate Bayesian inference algorithm for estimating the parameters of a nonlinear function from a potentially non-stationary data stream. The method is based on the extended Kalman filter (EKF), but uses a novel low-rank plus diagonal decomposition of the posterior precision matrix, which gives a cost per step which is linear in the number of model parameters. In contrast to methods based on stochastic variational inference, our method is fully deterministic, and does not require step-size tuning. We show experimentally that this results in much faster (more sample efficient) learning, which results in more rapid adaptation to changing distributions, and faster accumulation of reward when used as part of a contextual bandit algorithm.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> packages.tex <==

\newcommand{\myeat}[1]{}
%http://www.stackprinter.com/export?service=tex.stackexchange&question=59702&printer=false&linktohome=true

%\usepackage[framemethod=TikZ]{mdframed}

% https://tex.stackexchange.com/questions/99049/latex-error-option-clash-for-package-xcolor-even-if-i-put-listings-before
%https://en.wikibooks.org/wiki/LaTeX/Colors
\usepackage[usenames,dvipsnames]{xcolor}
%\usepackage[usenames]{color}

%\usepackage{float}
\usepackage{longtable}

\usepackage[toc,page]{appendix}

%\usepackage{tocloft}
%\advance\cftchapnumwidth 1cm
%https://tex.stackexchange.com/questions/436063/spacing-between-number-and-text-in-toc
%\advance\cftsecnumwidth 0.5em\relax


% https://mirror.las.iastate.edu/tex-archive/macros/latex/contrib/mathalpha/doc/mathalpha-doc.pdf
\usepackage{bm}
\usepackage{frcursive} 
\usepackage{xfrac}
\usepackage{mathrsfs}

\usepackage{fancyvrb} % https://tex.stackexchange.com/questions/122195/how-to-center-verbatim
\usepackage{xspace}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}

%https://tex.stackexchange.com/questions/58098/what-are-all-the-font-styles-i-can-use-in-math-mode
\usepackage[mathscr]{euscript}

\mathchardef\mhyphen="2D % Define a "math hyphen"
\mathchardef\mdash="2D % Define a "math hyphen"

%\usepackage{undertilde}
\usepackage{accents}


\usepackage[font={small,it}]{caption}
%\usepackage{subfigure}
\usepackage{subcaption} 
\usepackage{subfig}
%\usepackage{caption}
%\usepackage[font={small,it}]{subcaption} % https://en.wikibooks.org/wiki/LaTeX/Floats,_Figures_and_Captions#Subfloats

%https://tex.stackexchange.com/questions/283324/different-font-sizes-for-figure-and-subfigure-captions/283327
%\captionsetup{font={footnotesize,it}}
%\captionsetup[sub]{font={footnotesize,it}}

%\usepackage[font={small,it}]{caption}
%\usepackage[font={footnotesize,it}]{caption}

\usepackage{url}
\usepackage{cancel} % \cancel for strikethrough
\usepackage{multirow}
\usepackage{multicol}




\usepackage{verbatim}
%\usepackage{comment} %http://www.ctan.org/tex-archive/macros/latex/contrib/comment/

% From https://media.nips.cc/Conferences/NIPS2017/Styles/nips_2017.tex
% https://tex.stackexchange.com/questions/406179/how-to-type-the-letter-%C5%81

\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% https://tex.stackexchange.com/questions/392208/command-k-unavailable-in-encoding-ot1-error-takes-me-to-line-which-doesnt-eve

%http://mirrors.ibiblio.org/CTAN/macros/latex/base/utf8ienc.pdf
\usepackage[utf8]{inputenc}
%\DeclareUnicodeCharacter{2010}{-}% support older LaTeX versions
%\DeclareUnicodeCharacter{2212}{-}% support older LaTeX versions
%\DeclareUnicodeCharacter{301}{-}% support older LaTeX versions
%\DeclareUnicodeCharacter{00B4}{\textasciiacute}
\DeclareUnicodeCharacter{00B4}{'}


\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography



%https://tex.stackexchange.com/questions/36660/only-authors-initials-in-bibtex-natbib-using-named-style

%http://mirrors.ibiblio.org/CTAN/macros/latex/exptl/biblatex/doc/biblatex.pdf
%  bibstyle=authortitle,
\usepackage[
  style=alphabetic,
  citestyle=alphabetic,
  natbib=true,
  backend=bibtex,
  maxcitenames=3,  mincitenames=1,
  maxbibnames=10,  minbibnames=1,
  firstinits=true,
  backref=false, 
  hyperref=true,
  doi=false,  isbn=false,  url=false,
  arxiv=abs
]{biblatex}

%https://tex.stackexchange.com/questions/36307/formatting-back-references-in-bibliography
\DefineBibliographyStrings{english}{%
  backrefpage = {page},% originally "cited on page"
  backrefpages = {pages},% originally "cited on pages"
}

\usepackage{xpatch}

\usepackage{booktabs}
\usepackage{comment}

\usepackage{paralist} % compactenunm, compactitem

\usepackage{tikz}
\usetikzlibrary{fit,arrows,calc,positioning,shadows.blur}

% https://www.overleaf.com/learn/how-to/Cross_referencing_with_the_xr_package_in_Overleaf
%https://tex.stackexchange.com/questions/14364/cross-referencing-between-different-files?noredirect=1&lq=1
%https://texfaq.org/FAQ-extref
\usepackage{xr}
%\usepackage{xr-hyper}
%\usepackage{zref-xr,zref-user}

%\externaldocument{app}


% From 	Mykel Kochenderfer 
\usepackage{mathtools}
\DeclarePairedDelimiter{\paren}{\lparen}{\rparen}
\DeclarePairedDelimiter{\brock}{\lbrack}{\rbrack}

\usepackage{enumitem}


%\usepackage{algorithm}
%\usepackage{algpseudocode}

% https://jdhao.github.io/2019/09/21/latex_algorithm_pseudo_code/

\usepackage[ruled,vlined,linesnumbered,algochapter]{algorithm2e}
%\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
%\usepackage[noend]{algpseudocode}
%\usepackage{algorithmic}
\DontPrintSemicolon
\newcommand{\dontprintsemicolon}{}
% https://tex.stackexchange.com/questions/192435/adding-a-blank-line-in-algorithm2e

\usepackage{mdframed}
\usepackage{multicol}
\usepackage{rotating}
\usepackage{setspace}



\usepackage{blkarray}



%https://www.tug.org/FontCatalogue/newpx/
%https://wiki.carleton.edu/download/attachments/20155418/fontguide.pdf?version=1&modificationDate=1388599695000&api=v2
%\usepackage{newpxmath,newpxtext}

% https://tex.stackexchange.com/questions/514149/three-column-full-page-index-in-tufte-booktwoside-symmetric
%\usepackage[makeindex]{imakeidx}
\usepackage{imakeidx}
\usepackage[columns=3]{idxlayout}

% Hyperref needs to be last package
%https://tex.stackexchange.com/questions/326950/hyperref-conflicts-with-footnotea
%\usepackage[pagebackref=true,colorlinks=true,pdftex]{hyperref} % incompatible
%\usepackage[backref=true,colorlinks=true,pdftex]{hyperref} % incompatible

% https://tex.stackexchange.com/questions/35422/partition-numbering-and-pdf-bookmark-generation/35430#35430
\usepackage[bookmarksnumbered]{hyperref}

%\hypersetup{hidelinks,backref=true,pagebackref=true,hyperindex=true,hypertexnames=false,colorlinks=false,breaklinks=true,bookmarks=true,bookmarksopen=false,pdftitle={Title},pdfauthor={Author}}



\usepackage[capitalize]{cleveref}
%\usepackage{cleveref}
\Crefname{equation}{Equation}{Equations}
\crefname{equation}{Equation}{Equations}
\Crefname{section}{Section}{Sections}
\crefname{section}{Section}{Sections}
\Crefname{chapter}{Chapter}{Chapters}
\crefname{chapter}{Chapter}{Chapters}
\Crefname{figure}{Figure}{Figures}
\crefname{figure}{Figure}{Figures}
\Crefname{appsec}{Appendix}{Appendices}
\crefname{appsec}{Appendix}{Appendices}
%\usepackage[noabbrev,capitalize,nameinlink]{cleveref}


%https://robjhyndman.com/hyndsight/squeezing-space-with-latex/
%\usepackage{fontspec}
%setmonofont{DejaVu Sans Mono}[Scale=MatchLowercase]
%\setmainfont{DejaVu Sans}
%There is no ∇ (U+2207) in font ec-lmr10!

%http://www.gang.umass.edu/~franz/latexmanual.pdf


%https://image-color.com/color-picker#DA4F4F



\definecolor{cyan}{cmyk}{1,0,0,0.4}
\definecolor{magenta}{cmyk}{0,1,0,0.15}
\definecolor{yellow}{cmyk}{0,0,1,0}
\definecolor{black}{cmyk}{0,0,0,1}
\definecolor{orange}{cmyk}{0,0.5,1,0}
\definecolor{red}{cmyk}{0.00,0.92,0.92,0.06}
\definecolor{blue}{cmyk}{0.92,0.92,0.00,0.06}
\definecolor{green}{cmyk}{0.88,0.00,0.78,0.03}

\hypersetup{
    colorlinks,
    citecolor=magenta,
    linkcolor=magenta,
    urlcolor=cyan,
}

\usepackage{eqnalign}
\usepackage{version}

% Provide toggle to enable if..else conditions
\usepackage{etoolbox}


==> sections/iekf.tex <==
\subsection{Iterated EKF}

The iterated EKF is a simple extension of the EKF where the update step is iterated multiple times, so that the observation model can be relinearized at the current posterior
mean state estimate.
This can be further improved by adding a line search, to ensure that the updates improve the corresponding quadratic energy function, as explained in 
\citep{Skoglund2015}.
The resulting algorithm is much more stable than standard (I)EKF.
We give the pseudocode for the IEKF
in \cref{algo:IEFK}.
This can be extended to \lofi as shown in 
\cref{algo:ILOFI}.



\begin{algorithm}
def $\text{Iterated-EKF-update}(\vmu_{t|t-1}, \vSigma_{t|t-1}^{-1},
\vx_t, \vy_t, \vR_t, N)$
\\
$\vA_t = \text{chol}(\vR_t^{-1})$ \\
$\vSigma_{t|t-1}^{-\half} =
\text{chol}(\vSigma_{t|t-1}^{-1})$ \\
$\vSigma_{t|t-1} = \text{inv}(\vSigma_{t|t-1}^{-1})$ \\
$\vmu_1 = \vmu_{t|t-1}$ \\
\For{$i=1:N$}{
$\vH_i = \text{jac}(h(\vx_t,\cdot))(\vmu_i)$ \\
$\vS_i = \vH_i \vSigma_{t|t-1} \vH_i^\trans + \vR_t$ \\ 
$\vK_i = \vSigma_{t|t-1} \vH_i^\trans \vS_i^{-1}$ \\
$\hat{\vy}_i = h(\vx_t,\vmu_i) + \vH_i(\vmu_{t|t-1} - \vmu_i)$\\
$\vdelta_i = \vmu_{t|t-1} - \vmu_i 
+ \vK_i(\vy_t - \hat{\vy}_i)$ \\
$\alpha_i = \text{linesearch}(\vdelta_i,
\vmu_{t|t-1}, \vSigma_{t|t-1}^{-\half},
\vA_t,  \vx_t
)$ \\
$\vmu_{i+1} = \vmu_{i} + \alpha_i \vdelta_i$
}
$\vmu_{t|t} = \vmu_N$\\
%$\vSigma_{t|t} = (\vI - \vK_N \vH_N) \vSigma_{t|t-1}$\\
$\vSigma_{t|t}^{-1} =  \vSigma_{t|t-1}^{-1}
+ \vH_N^\trans \vR_t^{-1} \vH_N$\\
Return $(\vmu_{t|t}, \vSigma_{t|t}^{-1})$
\caption{Iterated EKF with linesearch}
\label{algo:IEFK}
\end{algorithm}


\begin{algorithm}
def $\text{Iterated-LOFI-update}(\vmu_{t|t-1}, 
\vU_{t|t-1}, \vlambda_{t|t-1}, \eta_{t|t-1}, 
\vx_t, \vy_t, \Var[\vy |\cdot], \memory, N)$
\\
$\hat{\vy}_t = h(\vx_t, \vmu_{t|t-1})$\\
$\vR_t = \Var[\vy \vert \hat{\vy_t}]$\\
$\vA_t = \text{chol}(\vR_t^{-1})$ \\
$\vSigma_{t|t-1}^{-\half} =
    \eta_{t|t-1}^{\half} \vI + 
     \sizeparam{\vU}_{t|t-1} 
    \diag( \vlambda_{t|t-1} )
    \sizeparam{\vU}_{t|t-1}^\trans$
  \\ 
$\vmu_1 = \vmu_{t|t-1}$ \\
\For{$i=1:N$}{
$\vH_i = \text{jac}(h(\vx_t,\cdot))(\vmu_i)$
\\
$\sizeout{\vW}_{i} \leftarrow \left[\begin{array}{cc}
\vU_{t | t-1} \diag(\vlambda_{t|t-1}) 
& \vH_{i}^{\trans} \vA_{t}^{\trans}
\end{array}\right]$
\\
$(\sizeout{\vU}_i, \sizeout{\vLambda}_i) = \text{SVD-full}(\sizeout{\vW}_i)$
\\
$\vD_{i} = \diag\left(
\frac{\sizeout{\vLambda}^2_{i}}
{\eta_{t|t-1}(\eta_{t|t-1}+\sizeout{\vLambda}^2_{i})}
\right)$
\\
$\vK_i = (\eta_{t|t-1}^{-1} \vI_\nparams
    - \sizeout{\vU}_{i}  \vD_{i} \sizeout{\vU}_{i}^\trans) \vH_i^\trans \vR_t^{-1}$
\\
$\hat{\vy}_i = h(\vx_t,\vmu_i) + \vH_i(\vmu_{t|t-1} - \vmu_i)$\\
$\vdelta_i = \vmu_{t|t-1} - \vmu_i 
+ \vK_i(\vy_t - \hat{\vy}_i)$ \\
$\alpha_i = \text{linesearch}(\vdelta_i,
\vmu_{t|t-1}, \vSigma_{t|t-1}^{-\half},
\vA_t,  \vx_t
)$ \\
$\vmu_{i+1} = \vmu_{i} + \alpha_i \vdelta_i$
}
$\vmu_{t|t} = \vmu_N$\\
%$\vSigma_{t|t} = (\vI - \vK_N \vH_N) \vSigma_{t|t-1}$\\
$(\vU_{t|t}, \vlambda_{t|t}) = \text{top-M}(\sizeout{\vU}_N, \sizeout{\vLambda}_N)$ \\
$\eta_{t|t} = \eta_{t|t-1}$ \\
Return $(\vmu_{t|t}, \vU_{t|t}, \vlambda_{t|t}, \eta_{t|t})$
\caption{Iterated LOFI with linesearch}
\label{algo:ILOFI}
\end{algorithm}

\begin{algorithm}
def linesearch($\vdelta_i,
\vmu_{t|t-1}, \vSigma_{t|t-1}^{-\half},
\vR_t^{-\half},  \vx_t)$: \\
Let $\cost(\vmu) = \half \vr(\vmu)^\trans \vr(\vmu)$
where
$\vr(\vmu) = \begin{pmatrix}
\vR_t^{-\half}(\vy_t - h(\vx_t,\vmu)) \\
\vSigma_{t|t-1}^{-\half} (\vmu_{t|t-1} - \vmu)
\end{pmatrix}$ 
\\
$\alpha_i = 1$\\
$\vmu_i = \vmu_{t|t-1} + \alpha_i \vdelta_i$\\
\eIf{$\cost(\vmu_i) < 
\cost(\vmu_{t|t-1})$}
{
Return $\alpha=1$
}
{
Return $\argmin_{0 < \alpha < 1} 
\cost(\vmu_{t|t-1} + \alpha \vdelta_i)$
} 
\caption{IEKF helper functions.}
\label{algo:IEFK-helper}
\end{algorithm}






==> sections/old-algo.tex <==


\eat{
% Version with W instead of U, Lambda
\begin{algorithm}
def $\text{predict}(
\vmu_{t-1}, \vUpsilon_{t-1}, \vW_{t-1}, \vx_t, \gamma_t, q_t)$: 
\\
$\vW_{t-1} = \vU_{t-1} \vLambda_{t-1}$
// Recreate the prior low-rank precision \\
$\vmu_{t|t-1} = \gamma \vmu_{t-1}$
// Predict the next mean \\
\\
$\vUpsilon_{t|t-1} = 
    \left(\gamma_t^{2} \vUpsilon_{t-1}^{-1}
    +q_t\vI_\nparams\right)^{-1}$
    \label{eq:LOFI-gen-diagonal-predict}
    // Predict the next diagonal precision 
\\
$\vC_t = 
\left(
            \vI_{\memory}
            + q_t \vW_{t-1}^{\trans}  \vUpsilon_{t|t-1} \vUpsilon_{t-1}^{-1} \vW_{t-1}
        \right)^{-1}$
    \\
$\vW_{t|t-1} =
    \gamma_t  \vUpsilon_{t|t-1} \vUpsilon_{t-1}^{-1} \vW_{t-1} 
    {\rm chol}(\vC_t)$
    // Predict the next low-rank precision
     \label{eq:LOFI-gen-lowrank-predict}
\\
%$(\vLambda_{t|t-1},\vU_{t|t-1}) = {\rm SVD}(\vW_{t|t-1})$
%\label{line:SVD-predict-step}
%\\
$\hat{\vy}_t =
h\left(\vx_t, \vmu_{t|t-1} \right)$ 
// Predict the mean of the output 
\\
Return $(\hat{\vy}_t,  \vmu_{t|t-1}, \vUpsilon_{t|t-1}, 
\vW_{t|t-1})$ 
\caption{\lofi predict step}
\label{algo:LOFI-predict}
\end{algorithm}
}

\eat{
\algorithmfootnote{Note:
This algorithm matches \cref{algo:LOFI-predict} except for taking $\vLambda,\vU$ instead of $\vW$ as input and output, for compatibility with the code for spherical \lofi (see \cref{appx:spherical}). This change entails insertion of \cref{line:SVD-predict-step}, which otherwise is not necessary, as we could pass $\vW_{t|t-1}$ directly to \cref{algo:LOFI-update-UL}. Another option would be to define $\vU_{t|t-1}=\vW_{t|t-1}$ and $\vLambda_{t|t-1}=\vI_\memory$ since \cref{algo:LOFI-update-UL} uses only the product $\vU_{t|t-1}\vLambda_{t|t-1}$, but we have left it written as is for conceptual clarity.
}
}


\eat{
% Version with W instead of U, Lambda
\begin{algorithm}
def $\text{update}(
\vmu_{t|t-1}, \vUpsilon_{t|t-1}, \vW_{t|t-1},
\vx_t, \vy_t, \hat{\vy}_t, \Var[\vy |\cdot], \memory)$: 
\\
$\ve_t = \vy_t - \hat{\vy}_t$ 
\\
$\vR_t = \Var[\vy \vert \hat{\vy_t}]$
\\
$\vA_t^\trans = \chol(\vR_t^{-1})$ 
\\
$\vH_t = \text{jac}(h(\vx_t,\cdot))(\vmu_{t|t-1})$
\\
$\sizeout{\vW}_{t} = \left[\begin{array}{cc}
    \vW_{t | t-1}
    & \vH_{t}^{\trans} \vA_{t}^{\trans}
    \end{array}\right]$
\\
$\vmu_{t}=\vmu_{t|t-1}+\left(\vUpsilon_{t|t-1}^{-1}-\vUpsilon_{t|t-1}^{-1}\sizeout{\vW}_{t}\left(\vI_{\memoryout}+\sizeout{\vW}_{t}^{\trans}\vUpsilon_{t|t-1}^{-1}\sizeout{\vW}_{t}\right)^{-1}\sizeout{\vW}_{t}^{\trans}\vUpsilon_{t|t-1}^{-1}\right)\vH_{t}^{\trans}\vR_{t}^{-1}\ve_{t}$
\\
$(\sizeout{\vLambda}_t,\sizeout{\vU}_t) = {\rm SVD}(\sizeout{\vW}_t)$ \\
$(\vLambda_{t}, \vU_{t}) = 
    \left(\sizeout{\vLambda}_t, \sizeout{\vU}_t\right)[:,1{:}\memory] $
\\
$\vW_t = \vU_t \vLambda_t$ \\
$(\vLambda_t^\times, \vU_t^\times) = 
    \left(\sizeout{\vLambda}_t, \sizeout{\vU}_t\right)[:,(\memory+1){:}\memoryout] $
\\
$\vW_t^{\times} = \vU_t^{\times} \vLambda_t^{\times}$ \\
$\vUpsilon_{t} =
    \vUpsilon_{t|t-1} +
    \diag\left(\vW_t^{\times} (\vW_t^{\times})^{\trans} \right)$
\\
Return $(\vmu_t, \vUpsilon_t,  \vW_t)$ 
\caption{\lofi update step.}
\label{algo:LOFI-update}
\end{algorithm}
}



